Multimodal Deep Models for Predicting Affective Responses Evoked by Movies

The goal of this study is to develop and analyze multimodal models for predicting experienced affective responses of viewers watching movie clips. We develop hybrid multimodal prediction models based on both the video and audio of the clips. For the video content, we hypothesize that both image content and motion are crucial features for evoked emotion prediction. To capture such information, we extract features from RGB frames and optical flow using pre-trained neural networks. For the audio model, we compute an enhanced set of low-level descriptors including intensity, loudness, cepstrum, linear predictor coefficients, pitch and voice quality. Both visual and audio features are then concatenated to create audio-visual features, which are used to predict the evoked emotion. To classify the movie clips into the corresponding affective response categories, we propose two approaches based on deep neural network models. The first one is based on fully connected layers without memory on the time component, the second incorporates the sequential dependency with a long short-term memory recurrent neural network (LSTM). We perform a thorough analysis of the importance of each feature set. Our experiments reveal that in our set-up, predicting emotions at each time step independently gives slightly better accuracy performance than with the LSTM. Interestingly, we also observe that the optical flow is more informative than the RGB in videos, and overall, models using audio features are more accurate than those based on video features when making the final prediction of evoked emotions.

==> recycle_bin.tex <==
 \citet{kahou2016emonets} propose to predict emotion of people that are talking in a video by designing an approach that is specifically crafted for their application and ensembles models of trained on modalities. They build a predictor based on video frames using a CNN for emotion prediction of faces, a mouth model of the human subject in video based on K-Means built with features around the mounth, and an autoencoder to extract motion features, all fused with a support vector machine (SVM) classifier that predict the emotion label. Then they construct a deep belief network which is trained on audio features extracted via the YAAFE library~\cite{mathieu2010yaafe}. After that, a random search algorithm combines the outputs of all these models. \dorien{how do they perform, why do we need to futher work on this? what's the gap? }. An approach proposed by \cite{fan2016video} consist on a hybrid network combining a LSTM and a 3D convolutional network with a late fusion to recognise emotion in video. CNNs are used to extract features from individual video frames before passing them to a LSTM, while a 3D convolutional network is applied to model appearance and motion of video simultaneously.  Audio features extracted by OpenSMILE toolkit~\cite{eyben2013recent} are fed to a SVM with the linear kernel. This approach is more related to ours, as we also apply a LSTM on audio-visual features extracted using CNNs and OpenSMILE. Besides predicting emotion evoked by videos, we also perform a thorough analysis and provide valuable insight into which features are more important for such emotion prediction.According to our experimental results, the LSTM structure with sequential dependency of emotion does not add much to the performance. Another recent multimodal approach~\cite{zheng2018multimodal}, which was an entry to One-Minute-Gradual Emotion Challenge, also includes text, in addition to audio and video features to predict the emotion, yet it only benefits the arousal prediction and not the valence. They also use  OpenSMILE, and apply SoundNet architecture~\cite{aytar2016soundnet} for acoustic feature extraction. For video,  CNNs such as VGG~\cite{simonyan2014very}, GoogleNet~\cite{szegedy2015going}, HoloNet~\cite{yao2016holonet}, ResNet~\cite{he2016deep} and DenseNet~\cite{huang2017densely} are applied to extract  facial emotion features, however, VGG16 outperforms others on both arousal and valence on One-Minute-Gradual Emotion Challenge’s validation datasets. The facial emotion features extracted using VGG16 are passed to two models, the first one with LSTM and the other with multiple 1D-CNN with different filter size 
 
 Then, features are all concatenated and passed through a SVM classifier. VGG16 is used to extract visual features, which are then fed to the LSTM or 1D-CNN model before being passed through an attention model. 
% GR: TODO - check the comment

%-------------------------------------------------------------------------------------
% Our proposed models are explained in more details as the followings: 
%
%\begin{figure} %[H]    % [t]
%\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.9 \linewidth}{0pt}}
%   \includegraphics[width=0.9 \linewidth]{RGB_OF_Audio_LSTM.png}
%\end{center}
%   \caption{The multimodal approach for emotion classification using LSTM recurrent neural network.}
%\label{fig:RGB_OF_Audio_LSTM}
%\end{figure}
%

%--------------------------------------------------------------------------------
Optical flow
Optical flow estimation is one of the core problems in computer vision, which has many applications related to object tracking and action recognition. Many approaches, \eg, gradient-based methods~\cite{horn1981determining}~\cite{lucas1981iterative}, correlation-based methods~\cite{anandan1989computational}, spatio-temporal energy based methods~\cite{adelson1985spatiotemporal} and phase-based methods~\cite{gautama2002phase} have been developed to compute optical flow, however, one of disadvantages of these methods is the computational cost for real time applications. A novel approach for overcoming this drawback is using CNN framework to estimate optical flow. Dosovitskiy \etal~\cite{dosovitskiy2015flownet} propose two CNNs namely FlowNetS and FlowNetC to estimate optical flow from raw images, however, their performances are below expectation. A stack of several FlowNetS and FlowNetC networks called FlowNet 2.0, proposed by ~\citet{ilg2017flownet}, works much faster while it performs equally to other approaches. A recent method for optical flow estimation called PWC-Net was proposed by \citet{sun2018pwc} based on three principles including pyramidal processing, warping, and cost volume processing. PWC-Net outperforms FlowNet 2.0 in model size, running time and accuracy on the final pass of the MPI-Sintel dataset. 
% Clean pass, which contains shading, but no image degradations, and the Final pass, which additionally includes motion blur, defocus blur, and atmospheric effects, and corresponds to the final movie

One of outstanding applications of optical flow is a research of ~\citet{simonyan2014two}, in which the authors propose a two-stream ConvNet model including a spatial and temporal stream for action recognition in video. Spatial stream ConvNet works on single still video frames, while temporal stream ConvNet operates on multi-frame optical flow. Averaging and linear SVM are two fusion techniques used to fuse the softmax scores of the two networks.
%
Optical flow is also used by \citet{venugopalan2015sequence}, who propose a sequence-to-sequence model to generate captions for videos, where frames are input sequentially and words are generated sequentially. Pre-trained VGG-16 and AlexNet are used to extract features from RGB video frames and optical flow images respectively. The extracted features are then concatenated and fed to the LSTM model. The implementation of this model achieves good performance on the MSVD dataset and outperforms related works on MPII-MD dataset and M-VAD dataset. 



%-------------------------------------------------------------
 The basic architecture of an LSTM cell includes a cell $c_{t}$ remembering values over time and three gates: input gate $i_{t}$, forget gate $f_{t}$ and output gate $o_{t}$. The LSTM cell can be described using the following equations~\cite{donahue2015long}: 
%
\begin{align}
f_{t} &= \textit{sigmoid} \left( W_{xf} x_{t} + W_{hf} h_{t-1} + b_{f} \right) \label{eq:LSTM-cell-1} \\
i_{t} &= \textit{sigmoid} \left( W_{xi} x_{t} + W_{hi} h_{t-1} + b_{i} \right) \label{eq:LSTM-cell-2} \\
g_{t} &= \textit{tanh} \left( W_{xc} x_{t} + W_{hc} h_{t-1} + b_{c} \right) \label{eq:LSTM-cell-3} \\
c_{t} &= f_{t} \odot c_{t-1} + i_{t} \odot g_{t} \label{eq:LSTM-cell-4} \\
o_{t} &= \textit{sigmoid} \left( W_{xo} x_{t} + W_{ho} h_{t-1} + b_{o} \right) \label{eq:LSTM-cell-5} \\
h_{t} &= o_{t} \odot \textit{tanh} \left( c_{t} \right) \label{eq:LSTM-cell-6} 
\end{align}
%
in which $x_{t}$ is the input ($t = 1, \dots, T$),  $T$ is the input sequence length, $h_{t} \in \mathbb{R}^{N}$ is the hidden state with $N$ being the number of hidden units; $ W_{xf}$, $ W_{hf}$, $W_{xi}$, $W_{hi}$, $W_{xc}$, $W_{hc}$, $W_{xo}$ and $W_{ho}$ are matrices of weights; $b_{f}$, $b_{i}$, $b_{c}$ and $b_{o}$ are biases; $\textit{sigmoid}$ is the sigmoid function $sigmoid (x) = \frac{1}{1+e^{-x}}$; $\odot$ is element-wise product.
%
The forget gate is the first and most important gate, which resets the LSTM cell state using a sigmoid function (equation \ref{eq:LSTM-cell-1}). The input gate decides which values will be updated using a sigmoid function  (equation \ref{eq:LSTM-cell-2}), and a $\tanh$ function is used to create a vector $g_{t}$ of new updated values (equation \ref{eq:LSTM-cell-3}). The cell state is computed from the forget gate, the previous cell state, input gate and the vector of new updated values (equation \ref{eq:LSTM-cell-4}). At the output gate, a sigmoid function is used to decide which part of the cell state is going to be the final output (equation \ref{eq:LSTM-cell-5}). The cell state is put through a $\tanh$ function to convert the values into the range $\left[ -1, 1 \right]$ and multiplied by the output (equation \ref{eq:LSTM-cell-6}). 
%
